A Multi-Domain Feature Learning Method for Visual Place Recognition

Visual Place Recognition (VPR) is an important component in both computer vision and robotics applications, thanks to its ability to determine whether a place has been visited and where specifically. A major challenge in VPR is to handle changes of environmental conditions including weather, season and illumination. Most VPR methods try to improve the place recognition performance by ignoring the environmental factors, leading to decreased accuracy decreases when environmental conditions change significantly, such as day versus night. To this end, we propose an end-to-end conditional visual place recognition method. Specifically, we introduce the multi-domain feature learning method (MDFL) to capture multiple attribute-descriptions for a given place, and then use a feature detaching module to separate the environmental condition-related features from those that are not. The only label required within this feature learning pipeline is the environmental condition. Evaluation of the proposed method is conducted on the multi-season \textit{NORDLAND} dataset, and the multi-weather \textit{GTAV} dataset. Experimental results show that our method improves the feature robustness against variant environmental conditions.

==> docs/method/network.tex <==
% TODO need to change table format
\begin{table}[h]
	\renewcommand{\arraystretch}{1}
	\caption[m1]{Multi-domain feature learner Networks Configurations}
	\label{table2}
	\centering
	\begin{center}
		\begin{tabular}{ | c| c| c | c | c  |}
			\hline
			Layer  & filter/caps & strides & bn & act \\  \hline
			\multicolumn{5}{|c|}{Encoder Module (MDFC)} \\ \hline
			conv1  & 64x5x5 & 2       & Y  & LeakRelu\\  \hline
			conv2  & 128x5x5 & 2       & Y  & LeakRelu\\  \hline
			conv3  & 256x5x5 & 1       & Y  & LeakRelu\\  \hline
			Pcaps[1:N]  & 512x9x9 & 2   & Y  & -\\  \hline
			PrimaryCaps & 32x6x6x(8) & - & -  & -\\  \hline
			DigitCaps & 64x(16) & - & -  & -\\  \hline
			\multicolumn{5}{|c|}{Decoder Module (MDFS)} \\ \hline
			fc1    & 512    & -       & Y  & LeakyRelu\\  \hline
			fc2    & 1024    & -       & Y  & LeakyRelu\\  \hline
			fc3    & 64x8x4x4   & -       & Y  & LeakyRelu\\  \hline
			deconv1  & 256x5x5 & 2 & Y & LeakyRelu \\  \hline
			deconv2  & 128x5x5 & 2 & Y & LeakyRelu \\  \hline
			deconv3  & 64x5x5  & 2 & Y & LeakyRelu \\  \hline
			deconv3  & 3x5x5   & 2 & Y & Sigmoid \\  \hline
			\multicolumn{5}{|c|}{Discriminator Module (MDFS)} \\ \hline			
			conv1  & 64x5x5 & 2 & Y & LeakyRelu \\  \hline
			conv2  & 128x5x5 & 2 & Y & LeakyRelu \\  \hline
			conv3  & 256x5x5 & 2 & Y & LeakyRelu \\  \hline
			conv3  & 512x5x5 & 2 & Y & LeakyRelu  \\  \hline
			fc1    & 512    & -  & Y  & LeakyRelu\\  \hline
			fc2    & 1024   & -  & Y  & LeakyRelu\\  \hline
			fc3    & 1      & -  & Y  & Sigmoid\\  \hline
		\end{tabular}
	\end{center}
\end{table}


\subsection{Network Structure}
The network is a combination of an MDFC module, an MDFS module. The MDFC module can be seen as an encoder module which is a combination of three sub-modules, the multi-attribute extraction sub-module, linear transformation sub-module, and the dynamic routing sub-module which are shown in Fig.~\ref{MDFC}. In the dynamic routing layer, we use $N_{objects}=64$ clustered capsules to model the potential objects in the scene, and $D_{feature} = 16$, i.e. each capsule is a 16-dimensional vector which contain both geometric features and condition features. The dimension of condition features dataset-dependent (four for the \textit{Nordland} datasets representing the four seasons, and three for the \textit{GTAV} datasets representing three weather conditions. The MDFS module has basically a GAN structure i.e. contains a decoder and a descriminator as shown in Fig.~\ref{GeometryCapturing}. The networks details are shown in Table (\ref{table2}).




